Watts: Infrastructure for Open-Ended Learning

This paper proposes a framework called Watts for implementing, comparing, and recombining open-ended learning (OEL) algorithms. Motivated by modularity and algorithmic flexibility, Watts atomizes the components of OEL systems to promote the study of and direct comparisons between approaches. Examining implementations of three OEL algorithms, the paper introduces the modules of the framework. The hope is for Watts to enable benchmarking and to explore new types of OEL algorithms. The repo is available at \url{https://github.com/aadharna/watts}

==> authros.tex <==
\author{Aaron Dharna\\
New Jersey Institute of Technology\
\texttt{\{aadharna}@gmail.com}}}

\And
Ji Q. Ren \& Yevgeny LeNet \\
Department of Computational Neuroscience \\
University of the Witwatersrand \\
Joburg, South Africa \\
\texttt{\{robot,net\}@wits.ac.za} \\
\AND
Coauthor \\
Affiliation \\
Address \\
\texttt{email}
}


\author{Aaron Dharna \And Charlie Summers \And Rohin Dasari \And Julian Togelius \And Amy K. Hoover}

\author{
    Aaron Dharna\IEEEauthorrefmark{1}, Charlie Summers\IEEEauthorrefmark{2},  Rohin Dasari\IEEEauthorrefmark{3}, Julian Togelius\IEEEauthorrefmark{3}, Amy K Hoover\IEEEauthorrefmark{1}}\\\
    \IEEEauthorblockA{\IEEEauthorrefmark{1}New Jersey Institute of Technology, USA, aadharna@gmail.com}\\\
    \IEEEauthorblockA{\IEEEauthorrefmark{2}Columbia University, USA}\\\
    \IEEEauthorblockA{\IEEEauthorrefmark{3}New York University, USA
    }
}


\author{Aaron Dharna \\
New Jersey Institute of Technology \\
\texttt{aadharna@gmail.com}\\
\And
Charlie Summers \\
Columbia University \\
\texttt{cgs2161@columbia.edu}\\
\AND
Rohin  Dasari\\
New York University \\
\texttt{rd2893@nyu.edu}\\
\And
Julian Togelius \\
New York University \\
\texttt{julian@togelius.com}\\
\And
Amy K. Hoover \\
New Jersey Institute of Technology \\
\texttt{ahoover@njit.edu}\\
}


\pdfinfo{
/Title (Watts: Infrastructure for Open-Ended Learning)
/Author (Aaron Dharna, Charlie Summers, Rohin Dasari, Julian Togelius, Amy K Hoover)}




